Space-time formulation, discretization, and computational performance studies for phase-field fracture optimal control problems

The purpose of this work is the development of space-time discretization schemes for phase-field optimal control problems. Specifically in the optimal control minimization problem, a tracking-type cost functional is minimized to steer the crack via the phase-field variable into a desired pattern. To achieve such optimal solutions, Neumann type boundary conditions need to be determined. First, a time discretization of the forward problem is derived using a discontinuous Galerkin formulation. Here, a challenge is to include regularization terms and the crack irreversibility constraint. The optimal control setting is formulated by means of the Lagrangian approach from which the primal part, adjoint, tangent and adjoint Hessian are derived. Herein the overall Newton algorithm is based on a reduced approach by eliminating the state constraint, namely the displacement and phase-field unknowns, but keeping the control variable as the only unknown. From the low-order discontinuous Galerkin discretization, adjoint time-stepping schemes are finally obtained. Both our formulation and algorithmic developments are substantiated and illustrated with six numerical experiments.

==> math-fields.tex <==
% Math fields -- requires amsfonts

\newcommand{\field}{\mathbb}

% "natural" names
\newcommand{\complex}{\field{C}}
\newcommand{\quaternions}{\field{H}}
\newcommand{\naturals}{\field{N}}
\newcommand{\polynomials}{\field{P}}
\newcommand{\rationals}{\field{Q}}
\newcommand{\reals}{\field{R}}
\newcommand{\integers}{\field{Z}}

% alternative names
\newcommand{\numsetC}{\complex}
\newcommand{\numsetH}{\quaternions}
\newcommand{\numsetN}{\naturals}
\newcommand{\numsetQ}{\rationals}
\newcommand{\numsetR}{\reals}
\newcommand{\numsetZ}{\integers}

% short names
\makeatletter
\@ifundefined{C}{\newcommand{\C}{\complex}}
{\PackageInfo{math-fields}{Use \string\field{C} for complex numbers;
 \MessageBreak command \string\C\space already defined}{}}
\makeatother
\newcommand{\N}{\naturals}
\newcommand{\Q}{\rationals}
\newcommand{\R}{\reals}
\newcommand{\Z}{\integers}
\newcommand{\Poly}{\polynomials}% deprecated: NuMa scripts


==> math-std.tex <==
% Standard math definitions -- requires amsmath

\newcommand\const{\textup{const}}% Also defined in documentclass siamltex.
\newcommand\qtext{\quad\text}
\newcommand\textq[1]{\text{#1}\quad}
\newcommand\qtextq{\quad\textq}
\newcommand\st{\textup{s.t.}}
\newcommand\stq{\st\quad}
\newcommand\qst{\quad\st}
\newcommand\qstq{\qst\quad}

\makeatletter
\newcommand\fcdot{\,\cdot\,}
\newcommand\ifgiven[3]{\def\fc@rg{#1}\ifx\fc@rg\empty#3\else#2\fi}
\newcommand\fcarg[1]{\ifgiven{#1}\fc@rg\fcdot}
\makeatother
\newcommand\abs[1]{\lvert\fcarg{#1}\rvert}
\newcommand\Abs[1]{\left\lvert#1\right\rvert}
\newcommand\tfracabs[2]{\abs{#1}/\abs{#2}}
\newcommand\fracabs[2]{\frac{\abs{#1}}{\abs{#2}}}
\newcommand\fracAbs[2]{\frac{\Abs{#1}}{\Abs{#2}}}
\newcommand\tabsfrac\tfracabs
\newcommand\absfrac\fracabs
\newcommand\Absfrac\fracAbs
\newcommand\card\abs
\newcommand\Card\Abs
\newcommand\ceil[1]{\lceil\fcarg{#1}\rceil}
\newcommand\Ceil[1]{\left\lceil#1\right\rceil}
\newcommand\defsep\colon% alternative: \mid
\newcommand\defset[3][\defsep]{\set{#2#1#3}}
\newcommand\Defset[3][\defsep]{\Set{#2#1#3}}
\newcommand\EEmult\cdot% alternative: \times
\newcommand\EE[1][\EEmult]{#1 10^}
\newcommand\floor[1]{\lfloor\fcarg{#1}\rfloor}
\newcommand\Floor[1]{\left\lfloor#1\right\rfloor}
\newcommand\Inv[1]{#1^{-1}}
\newcommand\HInv[1]{#1\ihr}% hermitian inverse
\newcommand\TInv[1]{#1\itp}% transpose inverse
\newcommand\norm[2][]{\lVert\fcarg{#2}\rVert\optsb{#1}}
\newcommand\Norm[2][]{\left\lVert#2\right\rVert\optsb{#1}}
\newcommand\tfracnorm[3][]{\norm[#1]{#2}/\norm[#1]{#3}}
\newcommand\fracnorm[3][]{\frac{\norm[#1]{#2}}{\norm[#1]{#3}}}
\newcommand\fracNorm[3][]{\frac{\Norm[#1]{#2}}{\Norm[#1]{#3}}}
\newcommand\tnormfrac\tfracnorm
\newcommand\normfrac\fracnorm
\newcommand\Normfrac\fracNorm
\newcommand\tfracnormpow[4][]{\norm[#1]{#2}^{#4}/\norm[#1]{#3}^{#4}}
\newcommand\fracnormpow[4][]{\frac{\norm[#1]{#2}^{#4}}{\norm[#1]{#3}^{#4}}}
\newcommand\fracNormpow[4][]{\frac{\Norm[#1]{#2}^{#4}}{\Norm[#1]{#3}^{#4}}}
\newcommand\pfrac[2]{\frac{\partial#1}{\partial#2}}
\newcommand\ppfrac[3]{\pfrac{^2#1}{#2\partial#3}}
\newcommand\set[1]{\{#1\}}
\newcommand\Set[1]{\left\{#1\right\}}
\newcommand\snorm[2][]{\lvert\!\lvert\!\lvert
  \fcarg{#2}\rvert\!\rvert\!\rvert\optsb{#1}}
\newcommand\Snorm[2][]{\left\lvert\!\left\lvert\!\left\lvert
  #2\right\rvert\!\right\rvert\!\right\rvert\optsb{#1}}
\newcommand\sprod[3][]{\langle\fcarg{#2},\fcarg{#3}\rangle\optsb{#1}}
\newcommand\Sprod[3][]{\left\langle#2,#3\right\rangle\optsb{#1}}

\newcommand\hrchar{H}
\newcommand\tpchar{T}
\newcommand\hr{^\hrchar}% hermitian transpose
\newcommand\tp{^\tpchar}
\newcommand\ihr{^{-\hrchar}}
\newcommand\itp{^{-\tpchar}}
\newcommand\tadj[1]{\mskip#1\thinmuskip}% adjust space
\newcommand\hra[1][0]{^{\tadj{#1}\hrchar}}
\providecommand\tpa[1][0]{^{\tadj{#1}\tpchar}}% Conflict with siamart190516.cls.
\newcommand\ihra[1][0]{^{\tadj{#1}{-}\hrchar}}
\newcommand\itpa[1][0]{^{\tadj{#1}{-}\tpchar}}
\newcommand\tpfrac[2]{\tfrac{\partial#1}{\partial#2}}
\newcommand\tppfrac[3]{\tpfrac{^2#1}{#2\partial#3}}
\newcommand\without{\setminus\set}
\newcommand\Without{\setminus\Set}

\newcommand\lbound{-}
\newcommand\ubound{+}
\newcommand\splb{^{\lbound}}
\newcommand\spub{^{\ubound}}
\newcommand\sblb{_{\lbound}}
\newcommand\sbub{_{\ubound}}
\newcommand\bounds[1]{\ensuremath{[#1\splb,#1\spub]}}
\newcommand\Bounds[1]{\ensuremath{\left[#1\splb,#1\spub\right]}}

\newcommand\Strut{\rule[2.5555ex]{0pt}{0pt}}% ~1.1em
\newcommand\Hline{\hline\Strut}

\newcommand\optsb[1]{\ifgiven{#1}{_{#1}}{}}
\newcommand\optsp[1]{\ifgiven{#1}{^{#1}}{}}
\newcommand\optindex[1]{\ifgiven{#1}{,#1}{}}
\newcommand\optmathsb\optsb
\newcommand\optmathsp\optsp
\newcommand\opttextsb[1]{\optsb{\textup{#1}}}
\newcommand\opttextsp[1]{\optsp{\textup{#1}}}
\newcommand\optmathindex\optindex
\newcommand\opttextindex[1]{\optindex{\textup{#1}}}

\newcommand\define{\mathrel{{\mathop:}{=}}}
\newcommand\enifed{\mathrel{{=}{\mathop:}}}

